AR-MAP: Are Autoregressive Large Language Models Implicit Teachers for Diffusion Large Language Models?

Diffusion Large Language Models (DLLMs) have emerged as a powerful alternative to autoregressive models, enabling parallel token generation across multiple positions. However, preference alignment of DLLMs remains challenging due to high variance introduced by Evidence Lower Bound (ELBO)-based likelihood estimation. In this work, we propose AR-MAP, a novel transfer learning framework that leverages preference-aligned autoregressive LLMs (AR-LLMs) as implicit teachers for DLLM alignment. We reveal that DLLMs can effectively absorb alignment knowledge from AR-LLMs through simple weight scaling, exploiting the shared architectural structure between these divergent generation paradigms. Crucially, our approach circumvents the high variance and computational overhead of direct DLLM alignment and comprehensive experiments across diverse preference alignment tasks demonstrate that AR-MAP achieves competitive or superior performance compared to existing DLLM-specific alignment methods, achieving 69.08\% average score across all tasks and models. Our Code is available at https://github.com/AMAP-ML/AR-MAP.

==> statement.tex <==
\section*{Impact Statement}

This work advances the foundational understanding of knowledge transfer between divergent generative paradigms, specifically revealing the latent weight mapping between autoregressive and diffusion language models. 
By introducing \ourmethod, we provide a computationally efficient pathway to align diffusion models, mitigating the high carbon footprint and instability associated with training them from scratch. 
Our findings encourage the research community to explore cross-architecture synergy rather than viewing different generative models in isolation, fostering the development of greener, more accessible, and well-aligned AI systems.

==> table.tex <==
  \begin{table}[!tbp]
\centering
\small
\caption{\textbf{HippoVlog} performance comparison. A+V: Cross-modal (Audio+Visual) accuracy; A: Audio-only accuracy; V: Visual-only accuracy; S: Semantic understanding accuracy.}
% \vspace{-0.5em}
\setlength{\tabcolsep}{5.2pt}
\begin{tabular}{l ccccc}
\Xhline{1.2pt}
\multirow{-1}{*}{\makecell{\textbf{Models}}}
& \textbf{A+V} & \textbf{A} & \textbf{V} & \textbf{S} & \textbf{Average} \\
\Xhline{0.5pt}

\rowcolor[HTML]{F6FF99} \multicolumn{6}{c}{\textit{Vanilla MLLMs}}\\
\Xhline{0.5pt}
\textsc{Gemini-2.5-Pro} & 63.6 & 69.2 & 75.2 & 80.0 & 72.0 \\
\textsc{Qwen3-VL-8B}    & 69.2 & 73.6 & 74.0 & 80.8 & 74.4 \\

\Xhline{0.5pt}
\rowcolor[HTML]{A7E399} \multicolumn{6}{c}{\textit{Long-Video LLMs}}\\
\Xhline{0.5pt}
\textsc{VideoChat-Flash} & 56.4 & 60.8 & 59.2 & 55.6 & 58.0 \\
\textsc{Time-R1}         & 49.4 & 58.2 & 58.2 & 52.4 & 54.6 \\
\textsc{Video-RTS}       & 56.8 & 58.8 & 62.0 & 58.4 & 59.0 \\

\Xhline{0.5pt}
\rowcolor[HTML]{48B3AF} \multicolumn{6}{c}{\color{white}\textit{RAG \& Memory-Augmented Systems}}\\
\Xhline{0.5pt}
\textsc{LightRAG}  & 44.8 & 51.6 & 46.0 & 47.2 & 47.4 \\
\textsc{HippoRAG}  & 54.0 & 72.4 & 53.2 & 73.2 & 63.2 \\
\textsc{Video-RAG} & 63.6 & 63.2 & 64.8 & 68.8 & 65.1 \\
\textsc{EgoRAG}    & 47.6 & 64.8 & 53.2 & 64.4 & 57.5 \\
\textsc{Ego-R1}    & 52.0 & 57.2 & 58.8 & 67.2 & 58.8 \\
\textsc{HippoMM}   & 59.2 & 68.8 & 77.6 & 82.0 & 71.9 \\

\Xhline{0.5pt}
\rowcolor[HTML]{476EAE} \multicolumn{6}{c}{\color{white}\textit{Memory Agents}}\\
\Xhline{0.5pt}
\textsc{M3-Agent}   & 50.8 & 68.4 & 72.4 & 70.4 & 65.5 \\
\textsc{WorldMM-8B} & 65.2 & 69.6 & 73.6 & 70.4 & 69.7 \\
\ourmethod          & \textbf{71.6} & \textbf{70.4} & \textbf{70.8} & \textbf{88.8} & \textbf{75.4} \\

\Xhline{1.2pt}
\end{tabular}
\label{tab:hippovlog}
\vspace{-0.8em}
\end{table}
